Validating Multimedia Content Moderation Software via Semantic Fusion

The exponential growth of social media platforms, such as Facebook and TikTok, has revolutionized communication and content publication in human society. Users on these platforms can publish multimedia content that delivers information via the combination of text, audio, images, and video. Meanwhile, the multimedia content release facility has been increasingly exploited to propagate toxic content, such as hate speech, malicious advertisements, and pornography. To this end, content moderation software has been widely deployed on these platforms to detect and blocks toxic content. However, due to the complexity of content moderation models and the difficulty of understanding information across multiple modalities, existing content moderation software can fail to detect toxic content, which often leads to extremely negative impacts. We introduce Semantic Fusion, a general, effective methodology for validating multimedia content moderation software. Our key idea is to fuse two or more existing single-modal inputs (e.g., a textual sentence and an image) into a new input that combines the semantics of its ancestors in a novel manner and has toxic nature by construction. This fused input is then used for validating multimedia content moderation software. We realized Semantic Fusion as DUO, a practical content moderation software testing tool. In our evaluation, we employ DUO to test five commercial content moderation software and two state-of-the-art models against three kinds of toxic content. The results show that DUO achieves up to 100% error finding rate (EFR) when testing moderation software. In addition, we leverage the test cases generated by DUO to retrain the two models we explored, which largely improves model robustness while maintaining the accuracy on the original test set.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Sections/1_Introduction.tex <==
\section{Introduction}

\label{sec-introduction}
Multimedia contents, such as Internet meme and video, have become an important role in online communication and content publication on social media platforms.
For example, in 2020, at least one million posts mentioning "meme" were shared every day in Instagram, one of the most popular social media platforms~\cite{meme2022}. 
Moreover, Cisco reports that 82\% of global internet traffic will come from either video streaming or video downloads in 2022~\cite{video2022}. 
Although the exponential growth of Internet multimedia platform tremendously facilitates users’ communication and content publishing around the world, it exacerbates the propagation of toxic contents. 

Toxic contents generally refer to Textual toxic contents, which can be typically divided into three types: (1) \textit{abusive language and hate speech}, which are abusive texts targeting specific individuals, such as politicians, celebrities, religions, nations, and the LGBTIQA+~\cite{Badjatiya2017DeepLF}; (2) \textit{malicious advertisement}, which are online advertisements with illegal purposes, such as phishing and scam links, malware download, and illegal information dissemination~\cite{Li2012KnowingYE}; and (3) \textit{pornography}, which is often sexually explicit, associative, and aroused~\cite{Rowley2006LargeSI}.

Toxic contents have significant negative impacts on users.
For instance, Munro \cite{children2011} studied the ill-effects of online hate speech on children, concluding that children may develop depression, anxiety, and other mental health problems as a result of their encounters online. Moreover, from May 2019 to May 2020, adult content sites accounted for 0.67 \% of all website categories accessed by Latin American children \cite{porn2022}. Pornographic contents can cause significant undesirable effects on the physical and psychological health of children \cite{Yu2016InternetMI}. 
These problems greatly affect social harmony and increase the number of criminal cases to a certain extent \cite{Chen2020AutomaticDO}. 
Malicious advertisements can be exploited for illegal purposes, such as providing phishing and scam links, propagating malware, and disseminating illegal information \cite{Li2012KnowingYE}. Malicious advertisements also remain a global burden, accounting for up to 85\% of daily message traffic \cite{spam2022}.

\begin{figure}
    \centering
    %\hspace{0.1cm}
    \begin{minipage}[c]{0.16\textwidth} 
        \begin{subfigure}{\textwidth} 
          \centering 
          \includegraphics[width=\linewidth]{Figures/shit.png}
          %\vspace{-1.3em}
        \end{subfigure}%
    \end{minipage}
   % \hspace{0.1cm}
    \begin{minipage}[c]{0.22\textwidth} 
        \begin{subfigure}{\textwidth} 
          \centering 
          \includegraphics[width=\linewidth]{Figures/monkey.jpeg}
          %\vspace{-1.3em}
        \end{subfigure}% 
    \end{minipage}
    \caption{The example of multimedia images. These two figures can be counted as hateful if we replace "XXX" with a specific group (e.g., racial, gender, religion or nation) for the left and replace the figure with a photo of specific group for the right.}
    \label{fig:trans}
    %\vspace{-0.6em}
    \label{fig_example}
\end{figure}

As a result, content moderation software, which detects and blocks toxic contents, has attracted massive interests from both academia and industry. 
Researchers typically formulate toxic content detection as a classification task and leverage various deep learning models to perform classification, including convolutional neuron networks, long-short-term-memory models, and Transformer-based models \cite{Mishra2019TacklingOA, Schmidt2017ASO, Wu2018TwitterSD}. 
With the help of the above techniques, the held-out accuracy of toxic content detection has been improved significantly. The industrial companies, including Google, Facebook, Twitter, and Baidu \cite{google2021, facebook2020, twitter2020, notrobustbaidu}, have also extensively and enthusiastically deployed commercial-level content moderation software on their products.

However, multimedia content moderation is not an easy task. Different from textual content moderation, multimedia content moderation is more complicated since it needs to mine and fuse the information from different modalities. 
For example, Figure~\ref{fig_example} shows a memes/video with a photo of a group of black people with a text/narration saying "these are monkeys", which should be counted as racial discrimination and hate speech, even though neither the photo nor the text/narration is discriminatory when being considered alone. 
Unfortunately, existing mainstream content moderation software proposed by big companies still contain defects, thus causing severe results.
For example, a New Zealand terrorist live-streamed a massacre on Facebook~\cite{newzealand}. And YouTube Kids, an app supposedly designed for children, was discovered to contain a significant amount of inappropriate contents, which were made readily available for unsuspecting kids in 2017~\cite{detect_fail}. \jz{Hence, sota methods not effective.}

\jz{reliability. 2 challenges: case generation and oracle.}
In order to improve the robustness of content moderation software, generating diverse test cases is a first step. Unfortunately, previous studies mainly focus on certain modality, such as visual~\cite{Zaidan2015RobustPC}, audio~\cite{Ibaez2021AudioBasedHS} and textual~\cite{Rttger2021HateCheckFT,Rttger2022MultilingualHF}, which cannot identify and fix the defects on information fusion of multi-modal video moderation. To overcome the drawbacks, in this paper, we propose \methodname, a framework utilizing \textbf{M}etamorphic \textbf{T}esting to comprehensively test \textbf{M}ultimedia content \textbf{M}oderation software. 

\methodname is designed to generate test cases for three content moderation tasks (\ie hate and abuse detection, pornographic content detection and advertisement detection) in both English and Chinese, two widely-used languages in the world. 
Specifically, \methodname first generates seed toxic sentences based on a template and keyword filling method. Then 4 methods are designed to generate image and video test cases under the idea of distributing the information of seed sentences into the combination of different modalities. The generated test cases and the seed sentences are fed into content moderation software and model to get the predicted toxicity. Finally, \methodname detects and reports suspicious failures based on our metamorphic relation. 


We conducted extensive experiments to validate the performance \methodname. We utilize \methodname to test five widely-deployed commercial content moderation products from famous providers including Google Cloud, Amazon Web Service, Baidu Cloud, Tencent Cloud and Alibaba Cloud, as well as two state-of-the-art research models for multimedia content moderation (\ie Vision-Transformer-based and ResNet-based classification models). Experimental results show that, although all software under test perform well on original datasets, most of them fail to detect the test cases generated by \methodname. Notably, up to 100\% of toxic image and video can bypass the content moderation tools.

The contributions of this paper are summarized as follows:
\begin{itemize}[leftmargin=*]
\item We introduce the first metamorphic testing framework, namely \methodname, to test multimedia content moderation software. 
% 启发之后的test case generation
\item We comprehensively include image test cases and video test cases generation for three kinds of toxic contents in both English and Chinese.
% highlight效果 xxx\%
\item We leverage the test cases produced by our \methodname to test five widely-deployed commercial software products and two state-of-the-art research models for multimedia content moderation. 
% 通过重训提升了模型性能，说明了xxx工具的有效性
\item We further improve the robustness of content moderation models by adopting the failed test cases to perform model retraining.
\end{itemize}

\noindent \textbf{Content Warning}: We apologize that this article presents examples of aggressive, abusive, and pornographic expressions to demonstrate the results of our method. Examples are quoted verbatim. For the mental health of participating researchers, we prompted a content warning in every stage of this work to the researchers and annotators, and told them that they were free to leave anytime during the study. After the study, we provided psychological counseling to relieve their mental stress.


==> Sections/2_Background.tex <==
\section{Background}
\label{sec-backgound}
% background 太长了，不相关的内容放到related work.
\jz{TODO: 1) move the single-modal content moderation and metamorphic testing sub-sections to related work. 2) introduce multi-modal techniques used in methodology (e.g., distribution and fusion).}
\subsection{Multimedia and Multi-modal AI}

Multimedia is a form of communication that uses a combination of different content forms such as text, audio, images, animations, or video into a single presentation. In artificial intelligence, the model that can deal with such multimedia data is called multi-modal AI, and each channel is called a modality. There are two main issues in multi-modal AI, processing single modality and fusing information between different modalities.  Our work mainly involve  three modalities: visual, audio and textual. For example, a memes containing visual and textual information and a video may include visual, audio and textual. 

\subsection{Content Moderation on Single Modality}

There are generally two categories of research models for content moderation, feature engineering-based models and neural networks-based models. Feature engineering-based models work by manually designing features and using the features to train classification models to identify toxic contents. While neural networks-based method is training a neural network models in an end-to-end manner on huge amount of data set to detect toxicity, without the need of much human effort on feature engineering.


\subsubsection{Visual Content Moderation Models}. 

\noindent \textbf{Feature Engineering-Based Models}. Early works on toxic image detection mainly extract some pre-designed features and then train a machine learning classifier. For example, Shen~\cite{Shen2010API} computed color histograms to detect pornography images, depends on  the activity suspicion  that pixels in pornographic images are mostly skin. Zhang~\cite{Zhang2005SemisupervisedAH} extract the motion features and use a hidden Markov model (HMM) for video anomaly detection.

\noindent \textbf{Neural Networks-Based Models}. With the development of deep learning techniques and the building of big data set, the progress of image representation learning have motivated researchers to explore neural network-based models for visual content moderation. Moustafa~\cite{Moustafa2015ApplyingDL} adapted a CNN architectures for image classification to the pornographic video classification task. Each frames are input for classifying them in
porn or non-porn and then he integrating the final result for a video through a
majority voting process.

\subsubsection{Audio Content Moderation Models}.

\noindent \textbf{Feature Engineering-Based Models}. Zhang~\cite{Zhang2005SemisupervisedAH} extracted Mel-Frequency Cepstral Coefficients (MFCCs) feature and use a HMM to detect audio events. \cite{Shi2009ObjectionableAC} extract various audio features, including MFCC, mean of short-time zero-crossing rates(mSTZCR), mean of spectral centroid(
SC) and high short-time zero-crossing rates
ratio(HZCRR), and use in-class clustering for porno-sounds detection.


\noindent \textbf{Neural Networks-Based Models}.Gupta~\cite{Gupta2022ADIMAAD} utilized a bidirectional Gated Recurrent Units(GRU) and Long Short-Term Memory (LSTM) model to  detect abuse from multilingual audio. Recently researchers proposed a deep learning method that can detect the COVID-19 from breath and cough audio~\cite{Coppock2021EndtoendCN}.

\subsubsection{Textual Content Moderation Models}.


\noindent \textbf{Feature Engineering-Based Models}. Textual feature engineering method can be further divided into rule-based methods and computation-based methods. 

Rule-based methods are based on pre-defined rules or dictionaries. Spertus et al. \cite{Spertus1997SmokeyAR} employed 47 handcrafted linguistic rules to extract binary feature vectors and used a decision tree to detect toxic contents. Razavi et al. \cite{Razavi2010AAI} constructed an abusive language dictionary to extract lexicon-level features for abuse detection. Handcrafted rules and lexicons generalize well across data from different domains. However, they can hardly deal with implicit abuse and sarcasm. Besides, they are vulnerable to errors in spelling, punctuation, and grammar \cite{Wiegand2018InducingAL}. 

Computation-based methods leverage some statistics of the textual data. Yin~\cite{Yin2009DetectionOH} computed TF-IDF of words as features and used a linear SVM to detect online harassment. Salminen et al. \cite{Salminen2018AnatomyOO} used TF-IDF weighted n-grams to train an SVM model for hate speech detection. Computation-based methods require less human effort and are more robust to spelling, punctuation, and grammatical variations. Nevertheless, this kind of approach can only capture surface-level patterns, not deeper semantic properties \cite{Wiegand2018InducingAL}.

\noindent \textbf{Neural Networks-Based Models}. Advancements in text representation learning have supurred researchers to explore neural network-based models for textual content moderation. Djuric et al. \cite{Djuric2015HateSD} was the first to use neural networks to obtain surface-level representations and trained a logistic regression classifier to detect abusive language. Badjatiya et al. \cite{Badjatiya2017DeepLF} used GLoVe word embedding to extract text features and used a word-level LSTM to moderate textual content. With the help of the pre-training models, some researchers fine-tuned pre-trained models, like BERT \cite{Devlin2019BERTPO} or RoBERTa \cite{Liu2019RoBERTaAR}, on a downstream dataset and have achieved remarkable performance on textual content moderation tasks.

\subsection{Multi-Modal Fusion}

A meme or video has different modalities to express the information. Hence the information from different modality should be fused to get the fully understating, such as whether it is toxic or not for content moderation software.

The fusion of different modalities is generally performed at two levels: feature level and decision level. 

In the feature level fusion approach, the features extracted from different modality are first combined and then sent as input to a single analysis unit that performs the analysis task. 

In the decision level fusion approach, the analysis units first provide the local decisions  that are obtained based on individual features from different modalities. The local decisions are then combined using a decision fusion  unit to make a fused decision. The advantages of decision level fusion is it allows us to use the most suitable methods for analyzing each single modality. However, it failure to utilize the feature level correlation among modalities.

\subsection{Commercial Content Moderation Software}

Big companies, for example, Google, Facebook, Twitter, and Baidu, have developed and deployed commercial-level content moderation software on their products. According to the official technical documents, the backbone of their software is usually a complected engineering system containing neural network-based models and rule-based methods. For example, Baidu Commercial Content Moderation Software is powered by a deep neural network and a huge pre-defined banned word list. This kind of hybrid approach can leverage the best of different methods. Neural networks-based methods can effectively mine contexts and semantic information, while rule-based methods can easily implement user-defined functionality.



% 这一段感觉可以直接放到related work
\subsection{Metamorphic Testing}

Metamorphic testing \cite{Chen2020MetamorphicTA} is a widely used technique to generate test cases to detect software faults automatically. It can solve the test oracle problem via metamorphic relations. Specifically, metamorphic relations describe the relation between bug-free software’s outputs on a input sample and that transformed by a pre-defined rule. Therefore, given an input sample, metamorphic testing transforms it into a new test case via a pre-defined transformation rule. Then by checking whether the outputs of the software on this pair of input samples satisfy the expected relation, metamorphic testing can identify the software bugs.

Consider a famous example that a program computing $\sin x$. According to mathematical property, a metamorphic relation for sine functions is "$\sin (\pi-x) = \sin x$". Thus, even though the expected value of $\sin x_1$ for the source test case is not known, a follow-up test case $x_2 = \pi-x_1$ can be constructed. We can verify whether $\sin x_1 = \sin x_2$ without knowing the concrete values of either sine calculation. Any inconsistency indicates a failure~\cite{Segura2016ASO}.

Metamorphic testing has been recently used for testing machine learning software. These efforts mainly focus on defining modifications in the dataset that can generate test cases to verify the quality of the model under test. Chen et al. investigated the use of MT in bioinformatics applications  \cite{Chen2008AnIA}. Xie et al. \cite{Xie2011TestingAV} defined 11 MRs to test k-Nearest Neighbors and Naive Bayes algorithms. Dwarakanath et al. \cite{Dwarakanath2018IdentifyingIB} presented 8 MRs to test SVM-based and ResNet-based image classifiers. Zhang et al. \cite{Zhang2018DeepRoadGM} tested image-based autonomous driving systems by applying GANs to produce driving scenes with various weather conditions and checking the consistency of the system outputs.


==> Sections/6_Related_Work.tex <==
\section{Related Work}

\subsection{Robustness of AI Software}

Artificial Intelligence (AI) software has been widely adopted by many domains, such as autonomous driving and face recognition. However, AI software is not robust enough and can generate erroneous outputs that lead to fatal accidents \cite{notrobustself-driving,notrobusttesla}. To test the robustness of AI software, researchers have proposed a variety of methods to generate adversarial examples that can fool AI software~\cite{Carlini2016HiddenVC,Tu2021ExploringAR, Luo2021InteractivePF}. Meanwhile, researchers have also designed approaches to improve AI software’s robustness, for example, the robust training mechanisms~\cite{Madry2018TowardsDL}. 

AI software has also become adept at solving many NLP tasks , such as sentiment analysis~\cite{Zhang2017SentimentAA}, reading comprehension~\cite{Yu2018QANetCL}, and machine translation\cite{Bahdanau2015NeuralMT}. In recent years, inspired by the work on adversarial examples in the computer vision field,  NLP researchers have started exploring attack and defense techniques for various NLP software~\cite{Gupta2020MachineTT, He2021TestingMT}. Ribeiro et al.~\cite{Ribeiro2020BeyondAB} designed a behavioral testing method to test NLP software for sentiment analysis, duplicate question answering and machine comprehension. Li et al.~\cite{Li2020BERTATTACKAA} used deep learning models to generate test cases for deep-learning based NLP software.

Our paper studies the robustness of a widely-adopted AI software, multimedia content moderation software, which has not been explored by these papers. 
